Asymptotic preserving $P_N$ methods for haptotaxis equations

The so-called haptotaxis equation is a special class of transport equation that arises from models of biological cell movement along tissue fibers. This equation has an anisotropic advection-diffusion equation as its macroscopic limit. An up to second-order accurate asymptotic preserving method is developed for the haptotaxis equation in space dimension up to three. For this the micro-macro decomposition proposed by Lemou and Mieussens is generalized in the context of finite-volume schemes on staggered grids. The spurious modes that arise from this discretization can be eliminated by combining flux evaluations from different points in the right way. The velocity space is discretized by an arbitrary-order linear moment system ($P_N$).

==> figures/cmRdBur.tex <==
\pgfplotsset{
colormap={cmRdBu_r}{
rgb(000pt)=(0.019608,0.188235,0.380392);
rgb(001pt)=(0.023914,0.196540,0.391926);
rgb(002pt)=(0.028220,0.204844,0.403460);
rgb(003pt)=(0.032526,0.213149,0.414994);
rgb(004pt)=(0.036832,0.221453,0.426528);
rgb(005pt)=(0.041138,0.229758,0.438062);
rgb(006pt)=(0.045444,0.238062,0.449596);
rgb(007pt)=(0.049750,0.246367,0.461130);
rgb(008pt)=(0.054056,0.254671,0.472664);
rgb(009pt)=(0.058362,0.262976,0.484198);
rgb(010pt)=(0.062668,0.271280,0.495732);
rgb(011pt)=(0.066974,0.279585,0.507266);
rgb(012pt)=(0.071280,0.287889,0.518800);
rgb(013pt)=(0.075586,0.296194,0.530335);
rgb(014pt)=(0.079892,0.304498,0.541869);
rgb(015pt)=(0.084198,0.312803,0.553403);
rgb(016pt)=(0.088504,0.321107,0.564937);
rgb(017pt)=(0.092810,0.329412,0.576471);
rgb(018pt)=(0.097116,0.337716,0.588005);
rgb(019pt)=(0.101423,0.346021,0.599539);
rgb(020pt)=(0.105729,0.354325,0.611073);
rgb(021pt)=(0.110035,0.362630,0.622607);
rgb(022pt)=(0.114341,0.370934,0.634141);
rgb(023pt)=(0.118647,0.379239,0.645675);
rgb(024pt)=(0.122953,0.387543,0.657209);
rgb(025pt)=(0.127259,0.395848,0.668743);
rgb(026pt)=(0.132026,0.403460,0.676278);
rgb(027pt)=(0.137255,0.410381,0.679815);
rgb(028pt)=(0.142484,0.417301,0.683353);
rgb(029pt)=(0.147712,0.424221,0.686890);
rgb(030pt)=(0.152941,0.431142,0.690427);
rgb(031pt)=(0.158170,0.438062,0.693964);
rgb(032pt)=(0.163399,0.444983,0.697501);
rgb(033pt)=(0.168627,0.451903,0.701038);
rgb(034pt)=(0.173856,0.458824,0.704575);
rgb(035pt)=(0.179085,0.465744,0.708112);
rgb(036pt)=(0.184314,0.472664,0.711649);
rgb(037pt)=(0.189542,0.479585,0.715186);
rgb(038pt)=(0.194771,0.486505,0.718724);
rgb(039pt)=(0.200000,0.493426,0.722261);
rgb(040pt)=(0.205229,0.500346,0.725798);
rgb(041pt)=(0.210458,0.507266,0.729335);
rgb(042pt)=(0.215686,0.514187,0.732872);
rgb(043pt)=(0.220915,0.521107,0.736409);
rgb(044pt)=(0.226144,0.528028,0.739946);
rgb(045pt)=(0.231373,0.534948,0.743483);
rgb(046pt)=(0.236601,0.541869,0.747020);
rgb(047pt)=(0.241830,0.548789,0.750557);
rgb(048pt)=(0.247059,0.555709,0.754095);
rgb(049pt)=(0.252288,0.562630,0.757632);
rgb(050pt)=(0.257516,0.569550,0.761169);
rgb(051pt)=(0.262745,0.576471,0.764706);
rgb(052pt)=(0.274894,0.584160,0.768858);
rgb(053pt)=(0.287043,0.591849,0.773010);
rgb(054pt)=(0.299193,0.599539,0.777163);
rgb(055pt)=(0.311342,0.607228,0.781315);
rgb(056pt)=(0.323491,0.614917,0.785467);
rgb(057pt)=(0.335640,0.622607,0.789619);
rgb(058pt)=(0.347789,0.630296,0.793772);
rgb(059pt)=(0.359939,0.637985,0.797924);
rgb(060pt)=(0.372088,0.645675,0.802076);
rgb(061pt)=(0.384237,0.653364,0.806228);
rgb(062pt)=(0.396386,0.661053,0.810381);
rgb(063pt)=(0.408535,0.668743,0.814533);
rgb(064pt)=(0.420684,0.676432,0.818685);
rgb(065pt)=(0.432834,0.684122,0.822837);
rgb(066pt)=(0.444983,0.691811,0.826990);
rgb(067pt)=(0.457132,0.699500,0.831142);
rgb(068pt)=(0.469281,0.707190,0.835294);
rgb(069pt)=(0.481430,0.714879,0.839446);
rgb(070pt)=(0.493579,0.722568,0.843599);
rgb(071pt)=(0.505729,0.730258,0.847751);
rgb(072pt)=(0.517878,0.737947,0.851903);
rgb(073pt)=(0.530027,0.745636,0.856055);
rgb(074pt)=(0.542176,0.753326,0.860208);
rgb(075pt)=(0.554325,0.761015,0.864360);
rgb(076pt)=(0.566474,0.768704,0.868512);
rgb(077pt)=(0.577393,0.775010,0.871972);
rgb(078pt)=(0.587082,0.779931,0.874740);
rgb(079pt)=(0.596770,0.784852,0.877509);
rgb(080pt)=(0.606459,0.789773,0.880277);
rgb(081pt)=(0.616148,0.794694,0.883045);
rgb(082pt)=(0.625836,0.799616,0.885813);
rgb(083pt)=(0.635525,0.804537,0.888581);
rgb(084pt)=(0.645213,0.809458,0.891349);
rgb(085pt)=(0.654902,0.814379,0.894118);
rgb(086pt)=(0.664591,0.819300,0.896886);
rgb(087pt)=(0.674279,0.824221,0.899654);
rgb(088pt)=(0.683968,0.829143,0.902422);
rgb(089pt)=(0.693656,0.834064,0.905190);
rgb(090pt)=(0.703345,0.838985,0.907958);
rgb(091pt)=(0.713033,0.843906,0.910727);
rgb(092pt)=(0.722722,0.848827,0.913495);
rgb(093pt)=(0.732411,0.853749,0.916263);
rgb(094pt)=(0.742099,0.858670,0.919031);
rgb(095pt)=(0.751788,0.863591,0.921799);
rgb(096pt)=(0.761476,0.868512,0.924567);
rgb(097pt)=(0.771165,0.873433,0.927336);
rgb(098pt)=(0.780854,0.878354,0.930104);
rgb(099pt)=(0.790542,0.883276,0.932872);
rgb(100pt)=(0.800231,0.888197,0.935640);
rgb(101pt)=(0.809919,0.893118,0.938408);
rgb(102pt)=(0.819608,0.898039,0.941176);
rgb(103pt)=(0.825452,0.900807,0.942253);
rgb(104pt)=(0.831296,0.903576,0.943329);
rgb(105pt)=(0.837140,0.906344,0.944406);
rgb(106pt)=(0.842983,0.909112,0.945483);
rgb(107pt)=(0.848827,0.911880,0.946559);
rgb(108pt)=(0.854671,0.914648,0.947636);
rgb(109pt)=(0.860515,0.917416,0.948712);
rgb(110pt)=(0.866359,0.920185,0.949789);
rgb(111pt)=(0.872203,0.922953,0.950865);
rgb(112pt)=(0.878047,0.925721,0.951942);
rgb(113pt)=(0.883891,0.928489,0.953018);
rgb(114pt)=(0.889735,0.931257,0.954095);
rgb(115pt)=(0.895579,0.934025,0.955171);
rgb(116pt)=(0.901423,0.936794,0.956248);
rgb(117pt)=(0.907266,0.939562,0.957324);
rgb(118pt)=(0.913110,0.942330,0.958401);
rgb(119pt)=(0.918954,0.945098,0.959477);
rgb(120pt)=(0.924798,0.947866,0.960554);
rgb(121pt)=(0.930642,0.950634,0.961630);
rgb(122pt)=(0.936486,0.953403,0.962707);
rgb(123pt)=(0.942330,0.956171,0.963783);
rgb(124pt)=(0.948174,0.958939,0.964860);
rgb(125pt)=(0.954018,0.961707,0.965936);
rgb(126pt)=(0.959862,0.964475,0.967013);
rgb(127pt)=(0.965705,0.967243,0.968089);
rgb(128pt)=(0.969089,0.966474,0.964937);
rgb(129pt)=(0.970012,0.962168,0.957555);
rgb(130pt)=(0.970934,0.957862,0.950173);
rgb(131pt)=(0.971857,0.953556,0.942791);
rgb(132pt)=(0.972780,0.949250,0.935409);
rgb(133pt)=(0.973702,0.944944,0.928028);
rgb(134pt)=(0.974625,0.940638,0.920646);
rgb(135pt)=(0.975548,0.936332,0.913264);
rgb(136pt)=(0.976471,0.932026,0.905882);
rgb(137pt)=(0.977393,0.927720,0.898501);
rgb(138pt)=(0.978316,0.923414,0.891119);
rgb(139pt)=(0.979239,0.919108,0.883737);
rgb(140pt)=(0.980161,0.914802,0.876355);
rgb(141pt)=(0.981084,0.910496,0.868973);
rgb(142pt)=(0.982007,0.906190,0.861592);
rgb(143pt)=(0.982930,0.901884,0.854210);
rgb(144pt)=(0.983852,0.897578,0.846828);
rgb(145pt)=(0.984775,0.893272,0.839446);
rgb(146pt)=(0.985698,0.888966,0.832065);
rgb(147pt)=(0.986621,0.884660,0.824683);
rgb(148pt)=(0.987543,0.880354,0.817301);
rgb(149pt)=(0.988466,0.876048,0.809919);
rgb(150pt)=(0.989389,0.871742,0.802537);
rgb(151pt)=(0.990311,0.867436,0.795156);
rgb(152pt)=(0.991234,0.863130,0.787774);
rgb(153pt)=(0.992157,0.858824,0.780392);
rgb(154pt)=(0.990773,0.850519,0.769781);
rgb(155pt)=(0.989389,0.842215,0.759170);
rgb(156pt)=(0.988005,0.833910,0.748558);
rgb(157pt)=(0.986621,0.825606,0.737947);
rgb(158pt)=(0.985236,0.817301,0.727336);
rgb(159pt)=(0.983852,0.808997,0.716724);
rgb(160pt)=(0.982468,0.800692,0.706113);
rgb(161pt)=(0.981084,0.792388,0.695502);
rgb(162pt)=(0.979700,0.784083,0.684890);
rgb(163pt)=(0.978316,0.775779,0.674279);
rgb(164pt)=(0.976932,0.767474,0.663668);
rgb(165pt)=(0.975548,0.759170,0.653057);
rgb(166pt)=(0.974164,0.750865,0.642445);
rgb(167pt)=(0.972780,0.742561,0.631834);
rgb(168pt)=(0.971396,0.734256,0.621223);
rgb(169pt)=(0.970012,0.725952,0.610611);
rgb(170pt)=(0.968627,0.717647,0.600000);
rgb(171pt)=(0.967243,0.709343,0.589389);
rgb(172pt)=(0.965859,0.701038,0.578777);
rgb(173pt)=(0.964475,0.692734,0.568166);
rgb(174pt)=(0.963091,0.684429,0.557555);
rgb(175pt)=(0.961707,0.676125,0.546944);
rgb(176pt)=(0.960323,0.667820,0.536332);
rgb(177pt)=(0.958939,0.659516,0.525721);
rgb(178pt)=(0.957555,0.651211,0.515110);
rgb(179pt)=(0.954556,0.641753,0.505729);
rgb(180pt)=(0.949942,0.631142,0.497578);
rgb(181pt)=(0.945329,0.620531,0.489427);
rgb(182pt)=(0.940715,0.609919,0.481276);
rgb(183pt)=(0.936102,0.599308,0.473126);
rgb(184pt)=(0.931488,0.588697,0.464975);
rgb(185pt)=(0.926874,0.578085,0.456824);
rgb(186pt)=(0.922261,0.567474,0.448674);
rgb(187pt)=(0.917647,0.556863,0.440523);
rgb(188pt)=(0.913033,0.546251,0.432372);
rgb(189pt)=(0.908420,0.535640,0.424221);
rgb(190pt)=(0.903806,0.525029,0.416071);
rgb(191pt)=(0.899193,0.514418,0.407920);
rgb(192pt)=(0.894579,0.503806,0.399769);
rgb(193pt)=(0.889965,0.493195,0.391619);
rgb(194pt)=(0.885352,0.482584,0.383468);
rgb(195pt)=(0.880738,0.471972,0.375317);
rgb(196pt)=(0.876125,0.461361,0.367166);
rgb(197pt)=(0.871511,0.450750,0.359016);
rgb(198pt)=(0.866897,0.440138,0.350865);
rgb(199pt)=(0.862284,0.429527,0.342714);
rgb(200pt)=(0.857670,0.418916,0.334564);
rgb(201pt)=(0.853057,0.408305,0.326413);
rgb(202pt)=(0.848443,0.397693,0.318262);
rgb(203pt)=(0.843829,0.387082,0.310112);
rgb(204pt)=(0.839216,0.376471,0.301961);
rgb(205pt)=(0.833679,0.365398,0.296732);
rgb(206pt)=(0.828143,0.354325,0.291503);
rgb(207pt)=(0.822607,0.343253,0.286275);
rgb(208pt)=(0.817070,0.332180,0.281046);
rgb(209pt)=(0.811534,0.321107,0.275817);
rgb(210pt)=(0.805998,0.310035,0.270588);
rgb(211pt)=(0.800461,0.298962,0.265359);
rgb(212pt)=(0.794925,0.287889,0.260131);
rgb(213pt)=(0.789389,0.276817,0.254902);
rgb(214pt)=(0.783852,0.265744,0.249673);
rgb(215pt)=(0.778316,0.254671,0.244444);
rgb(216pt)=(0.772780,0.243599,0.239216);
rgb(217pt)=(0.767243,0.232526,0.233987);
rgb(218pt)=(0.761707,0.221453,0.228758);
rgb(219pt)=(0.756171,0.210381,0.223529);
rgb(220pt)=(0.750634,0.199308,0.218301);
rgb(221pt)=(0.745098,0.188235,0.213072);
rgb(222pt)=(0.739562,0.177163,0.207843);
rgb(223pt)=(0.734025,0.166090,0.202614);
rgb(224pt)=(0.728489,0.155017,0.197386);
rgb(225pt)=(0.722953,0.143945,0.192157);
rgb(226pt)=(0.717416,0.132872,0.186928);
rgb(227pt)=(0.711880,0.121799,0.181699);
rgb(228pt)=(0.706344,0.110727,0.176471);
rgb(229pt)=(0.700807,0.099654,0.171242);
rgb(230pt)=(0.692272,0.092272,0.167705);
rgb(231pt)=(0.680738,0.088581,0.165859);
rgb(232pt)=(0.669204,0.084890,0.164014);
rgb(233pt)=(0.657670,0.081200,0.162168);
rgb(234pt)=(0.646136,0.077509,0.160323);
rgb(235pt)=(0.634602,0.073818,0.158478);
rgb(236pt)=(0.623068,0.070127,0.156632);
rgb(237pt)=(0.611534,0.066436,0.154787);
rgb(238pt)=(0.600000,0.062745,0.152941);
rgb(239pt)=(0.588466,0.059054,0.151096);
rgb(240pt)=(0.576932,0.055363,0.149250);
rgb(241pt)=(0.565398,0.051672,0.147405);
rgb(242pt)=(0.553864,0.047982,0.145559);
rgb(243pt)=(0.542330,0.044291,0.143714);
rgb(244pt)=(0.530796,0.040600,0.141869);
rgb(245pt)=(0.519262,0.036909,0.140023);
rgb(246pt)=(0.507728,0.033218,0.138178);
rgb(247pt)=(0.496194,0.029527,0.136332);
rgb(248pt)=(0.484660,0.025836,0.134487);
rgb(249pt)=(0.473126,0.022145,0.132641);
rgb(250pt)=(0.461592,0.018454,0.130796);
rgb(251pt)=(0.450058,0.014764,0.128950);
rgb(252pt)=(0.438524,0.011073,0.127105);
rgb(253pt)=(0.426990,0.007382,0.125260);
rgb(254pt)=(0.415456,0.003691,0.123414);
rgb(255pt)=(0.403922,0.000000,0.121569);
}
}


==> figures/cmxray.tex <==
\pgfplotsset{
	colormap={cmxray}{
rgb(0pt)=(1.000000,1.000000,1.000000);
rgb(1pt)=(0.996078,0.996078,0.996078);
rgb(2pt)=(0.992157,0.992157,0.992157);
rgb(3pt)=(0.988235,0.988235,0.988235);
rgb(4pt)=(0.984314,0.984314,0.984314);
rgb(5pt)=(0.980392,0.980392,0.980392);
rgb(6pt)=(0.976471,0.976471,0.976471);
rgb(7pt)=(0.972549,0.972549,0.972549);
rgb(8pt)=(0.968627,0.968627,0.968627);
rgb(9pt)=(0.964706,0.964706,0.964706);
rgb(10pt)=(0.960784,0.960784,0.960784);
rgb(11pt)=(0.956863,0.956863,0.956863);
rgb(12pt)=(0.952941,0.952941,0.952941);
rgb(13pt)=(0.949020,0.949020,0.949020);
rgb(14pt)=(0.945098,0.945098,0.945098);
rgb(15pt)=(0.941176,0.941176,0.941176);
rgb(16pt)=(0.937255,0.937255,0.937255);
rgb(17pt)=(0.933333,0.933333,0.933333);
rgb(18pt)=(0.929412,0.929412,0.929412);
rgb(19pt)=(0.925490,0.925490,0.925490);
rgb(20pt)=(0.921569,0.921569,0.921569);
rgb(21pt)=(0.917647,0.917647,0.917647);
rgb(22pt)=(0.913725,0.913725,0.913725);
rgb(23pt)=(0.909804,0.909804,0.909804);
rgb(24pt)=(0.905882,0.905882,0.905882);
rgb(25pt)=(0.901961,0.901961,0.901961);
rgb(26pt)=(0.898039,0.898039,0.898039);
rgb(27pt)=(0.894118,0.894118,0.894118);
rgb(28pt)=(0.890196,0.890196,0.890196);
rgb(29pt)=(0.886275,0.886275,0.886275);
rgb(30pt)=(0.882353,0.882353,0.882353);
rgb(31pt)=(0.878431,0.878431,0.878431);
rgb(32pt)=(0.874510,0.874510,0.874510);
rgb(33pt)=(0.870588,0.870588,0.870588);
rgb(34pt)=(0.866667,0.866667,0.866667);
rgb(35pt)=(0.862745,0.862745,0.862745);
rgb(36pt)=(0.858824,0.858824,0.858824);
rgb(37pt)=(0.854902,0.854902,0.854902);
rgb(38pt)=(0.850980,0.850980,0.850980);
rgb(39pt)=(0.847059,0.847059,0.847059);
rgb(40pt)=(0.843137,0.843137,0.843137);
rgb(41pt)=(0.839216,0.839216,0.839216);
rgb(42pt)=(0.835294,0.835294,0.835294);
rgb(43pt)=(0.831373,0.831373,0.831373);
rgb(44pt)=(0.827451,0.827451,0.827451);
rgb(45pt)=(0.823529,0.823529,0.823529);
rgb(46pt)=(0.819608,0.819608,0.819608);
rgb(47pt)=(0.815686,0.815686,0.815686);
rgb(48pt)=(0.811765,0.811765,0.811765);
rgb(49pt)=(0.807843,0.807843,0.807843);
rgb(50pt)=(0.803922,0.803922,0.803922);
rgb(51pt)=(0.800000,0.800000,0.800000);
rgb(52pt)=(0.796078,0.796078,0.796078);
rgb(53pt)=(0.792157,0.792157,0.792157);
rgb(54pt)=(0.788235,0.788235,0.788235);
rgb(55pt)=(0.784314,0.784314,0.784314);
rgb(56pt)=(0.780392,0.780392,0.780392);
rgb(57pt)=(0.776471,0.776471,0.776471);
rgb(58pt)=(0.772549,0.772549,0.772549);
rgb(59pt)=(0.768627,0.768627,0.768627);
rgb(60pt)=(0.764706,0.764706,0.764706);
rgb(61pt)=(0.760784,0.760784,0.760784);
rgb(62pt)=(0.756863,0.756863,0.756863);
rgb(63pt)=(0.752941,0.752941,0.752941);
rgb(64pt)=(0.749020,0.749020,0.749020);
rgb(65pt)=(0.745098,0.745098,0.745098);
rgb(66pt)=(0.741176,0.741176,0.741176);
rgb(67pt)=(0.737255,0.737255,0.737255);
rgb(68pt)=(0.733333,0.733333,0.733333);
rgb(69pt)=(0.729412,0.729412,0.729412);
rgb(70pt)=(0.725490,0.725490,0.725490);
rgb(71pt)=(0.721569,0.721569,0.721569);
rgb(72pt)=(0.717647,0.717647,0.717647);
rgb(73pt)=(0.713725,0.713725,0.713725);
rgb(74pt)=(0.709804,0.709804,0.709804);
rgb(75pt)=(0.705882,0.705882,0.705882);
rgb(76pt)=(0.701961,0.701961,0.701961);
rgb(77pt)=(0.698039,0.698039,0.698039);
rgb(78pt)=(0.694118,0.694118,0.694118);
rgb(79pt)=(0.690196,0.690196,0.690196);
rgb(80pt)=(0.686275,0.686275,0.686275);
rgb(81pt)=(0.682353,0.682353,0.682353);
rgb(82pt)=(0.678431,0.678431,0.678431);
rgb(83pt)=(0.674510,0.674510,0.674510);
rgb(84pt)=(0.670588,0.670588,0.670588);
rgb(85pt)=(0.666667,0.666667,0.666667);
rgb(86pt)=(0.662745,0.662745,0.662745);
rgb(87pt)=(0.658824,0.658824,0.658824);
rgb(88pt)=(0.654902,0.654902,0.654902);
rgb(89pt)=(0.650980,0.650980,0.650980);
rgb(90pt)=(0.647059,0.647059,0.647059);
rgb(91pt)=(0.643137,0.643137,0.643137);
rgb(92pt)=(0.639216,0.639216,0.639216);
rgb(93pt)=(0.635294,0.635294,0.635294);
rgb(94pt)=(0.631373,0.631373,0.631373);
rgb(95pt)=(0.627451,0.627451,0.627451);
rgb(96pt)=(0.623529,0.623529,0.623529);
rgb(97pt)=(0.619608,0.619608,0.619608);
rgb(98pt)=(0.615686,0.615686,0.615686);
rgb(99pt)=(0.611765,0.611765,0.611765);
rgb(100pt)=(0.607843,0.607843,0.607843);
rgb(101pt)=(0.603922,0.603922,0.603922);
rgb(102pt)=(0.600000,0.600000,0.600000);
rgb(103pt)=(0.596078,0.596078,0.596078);
rgb(104pt)=(0.592157,0.592157,0.592157);
rgb(105pt)=(0.588235,0.588235,0.588235);
rgb(106pt)=(0.584314,0.584314,0.584314);
rgb(107pt)=(0.580392,0.580392,0.580392);
rgb(108pt)=(0.576471,0.576471,0.576471);
rgb(109pt)=(0.572549,0.572549,0.572549);
rgb(110pt)=(0.568627,0.568627,0.568627);
rgb(111pt)=(0.564706,0.564706,0.564706);
rgb(112pt)=(0.560784,0.560784,0.560784);
rgb(113pt)=(0.556863,0.556863,0.556863);
rgb(114pt)=(0.552941,0.552941,0.552941);
rgb(115pt)=(0.549020,0.549020,0.549020);
rgb(116pt)=(0.545098,0.545098,0.545098);
rgb(117pt)=(0.541176,0.541176,0.541176);
rgb(118pt)=(0.537255,0.537255,0.537255);
rgb(119pt)=(0.533333,0.533333,0.533333);
rgb(120pt)=(0.529412,0.529412,0.529412);
rgb(121pt)=(0.525490,0.525490,0.525490);
rgb(122pt)=(0.521569,0.521569,0.521569);
rgb(123pt)=(0.517647,0.517647,0.517647);
rgb(124pt)=(0.513725,0.513725,0.513725);
rgb(125pt)=(0.509804,0.509804,0.509804);
rgb(126pt)=(0.505882,0.505882,0.505882);
rgb(127pt)=(0.501961,0.501961,0.501961);
rgb(128pt)=(0.498039,0.498039,0.498039);
rgb(129pt)=(0.494118,0.494118,0.494118);
rgb(130pt)=(0.490196,0.490196,0.490196);
rgb(131pt)=(0.486275,0.486275,0.486275);
rgb(132pt)=(0.482353,0.482353,0.482353);
rgb(133pt)=(0.478431,0.478431,0.478431);
rgb(134pt)=(0.474510,0.474510,0.474510);
rgb(135pt)=(0.470588,0.470588,0.470588);
rgb(136pt)=(0.466667,0.466667,0.466667);
rgb(137pt)=(0.462745,0.462745,0.462745);
rgb(138pt)=(0.458824,0.458824,0.458824);
rgb(139pt)=(0.454902,0.454902,0.454902);
rgb(140pt)=(0.450980,0.450980,0.450980);
rgb(141pt)=(0.447059,0.447059,0.447059);
rgb(142pt)=(0.443137,0.443137,0.443137);
rgb(143pt)=(0.439216,0.439216,0.439216);
rgb(144pt)=(0.435294,0.435294,0.435294);
rgb(145pt)=(0.431373,0.431373,0.431373);
rgb(146pt)=(0.427451,0.427451,0.427451);
rgb(147pt)=(0.423529,0.423529,0.423529);
rgb(148pt)=(0.419608,0.419608,0.419608);
rgb(149pt)=(0.415686,0.415686,0.415686);
rgb(150pt)=(0.411765,0.411765,0.411765);
rgb(151pt)=(0.407843,0.407843,0.407843);
rgb(152pt)=(0.403922,0.403922,0.403922);
rgb(153pt)=(0.400000,0.400000,0.400000);
rgb(154pt)=(0.396078,0.396078,0.396078);
rgb(155pt)=(0.392157,0.392157,0.392157);
rgb(156pt)=(0.388235,0.388235,0.388235);
rgb(157pt)=(0.384314,0.384314,0.384314);
rgb(158pt)=(0.380392,0.380392,0.380392);
rgb(159pt)=(0.376471,0.376471,0.376471);
rgb(160pt)=(0.372549,0.372549,0.372549);
rgb(161pt)=(0.368627,0.368627,0.368627);
rgb(162pt)=(0.364706,0.364706,0.364706);
rgb(163pt)=(0.360784,0.360784,0.360784);
rgb(164pt)=(0.356863,0.356863,0.356863);
rgb(165pt)=(0.352941,0.352941,0.352941);
rgb(166pt)=(0.349020,0.349020,0.349020);
rgb(167pt)=(0.345098,0.345098,0.345098);
rgb(168pt)=(0.341176,0.341176,0.341176);
rgb(169pt)=(0.337255,0.337255,0.337255);
rgb(170pt)=(0.333333,0.333333,0.333333);
rgb(171pt)=(0.329412,0.329412,0.329412);
rgb(172pt)=(0.325490,0.325490,0.325490);
rgb(173pt)=(0.321569,0.321569,0.321569);
rgb(174pt)=(0.317647,0.317647,0.317647);
rgb(175pt)=(0.313725,0.313725,0.313725);
rgb(176pt)=(0.309804,0.309804,0.309804);
rgb(177pt)=(0.305882,0.305882,0.305882);
rgb(178pt)=(0.301961,0.301961,0.301961);
rgb(179pt)=(0.298039,0.298039,0.298039);
rgb(180pt)=(0.294118,0.294118,0.294118);
rgb(181pt)=(0.290196,0.290196,0.290196);
rgb(182pt)=(0.286275,0.286275,0.286275);
rgb(183pt)=(0.282353,0.282353,0.282353);
rgb(184pt)=(0.278431,0.278431,0.278431);
rgb(185pt)=(0.274510,0.274510,0.274510);
rgb(186pt)=(0.270588,0.270588,0.270588);
rgb(187pt)=(0.266667,0.266667,0.266667);
rgb(188pt)=(0.262745,0.262745,0.262745);
rgb(189pt)=(0.258824,0.258824,0.258824);
rgb(190pt)=(0.254902,0.254902,0.254902);
rgb(191pt)=(0.250980,0.250980,0.250980);
rgb(192pt)=(0.247059,0.247059,0.247059);
rgb(193pt)=(0.243137,0.243137,0.243137);
rgb(194pt)=(0.239216,0.239216,0.239216);
rgb(195pt)=(0.235294,0.235294,0.235294);
rgb(196pt)=(0.231373,0.231373,0.231373);
rgb(197pt)=(0.227451,0.227451,0.227451);
rgb(198pt)=(0.223529,0.223529,0.223529);
rgb(199pt)=(0.219608,0.219608,0.219608);
rgb(200pt)=(0.215686,0.215686,0.215686);
rgb(201pt)=(0.211765,0.211765,0.211765);
rgb(202pt)=(0.207843,0.207843,0.207843);
rgb(203pt)=(0.203922,0.203922,0.203922);
rgb(204pt)=(0.200000,0.200000,0.200000);
rgb(205pt)=(0.196078,0.196078,0.196078);
rgb(206pt)=(0.192157,0.192157,0.192157);
rgb(207pt)=(0.188235,0.188235,0.188235);
rgb(208pt)=(0.184314,0.184314,0.184314);
rgb(209pt)=(0.180392,0.180392,0.180392);
rgb(210pt)=(0.176471,0.176471,0.176471);
rgb(211pt)=(0.172549,0.172549,0.172549);
rgb(212pt)=(0.168627,0.168627,0.168627);
rgb(213pt)=(0.164706,0.164706,0.164706);
rgb(214pt)=(0.160784,0.160784,0.160784);
rgb(215pt)=(0.156863,0.156863,0.156863);
rgb(216pt)=(0.152941,0.152941,0.152941);
rgb(217pt)=(0.149020,0.149020,0.149020);
rgb(218pt)=(0.145098,0.145098,0.145098);
rgb(219pt)=(0.141176,0.141176,0.141176);
rgb(220pt)=(0.137255,0.137255,0.137255);
rgb(221pt)=(0.133333,0.133333,0.133333);
rgb(222pt)=(0.129412,0.129412,0.129412);
rgb(223pt)=(0.125490,0.125490,0.125490);
rgb(224pt)=(0.121569,0.121569,0.121569);
rgb(225pt)=(0.117647,0.117647,0.117647);
rgb(226pt)=(0.113725,0.113725,0.113725);
rgb(227pt)=(0.109804,0.109804,0.109804);
rgb(228pt)=(0.105882,0.105882,0.105882);
rgb(229pt)=(0.101961,0.101961,0.101961);
rgb(230pt)=(0.098039,0.098039,0.098039);
rgb(231pt)=(0.094118,0.094118,0.094118);
rgb(232pt)=(0.090196,0.090196,0.090196);
rgb(233pt)=(0.086275,0.086275,0.086275);
rgb(234pt)=(0.082353,0.082353,0.082353);
rgb(235pt)=(0.078431,0.078431,0.078431);
rgb(236pt)=(0.074510,0.074510,0.074510);
rgb(237pt)=(0.070588,0.070588,0.070588);
rgb(238pt)=(0.066667,0.066667,0.066667);
rgb(239pt)=(0.062745,0.062745,0.062745);
rgb(240pt)=(0.058824,0.058824,0.058824);
rgb(241pt)=(0.054902,0.054902,0.054902);
rgb(242pt)=(0.050980,0.050980,0.050980);
rgb(243pt)=(0.047059,0.047059,0.047059);
rgb(244pt)=(0.043137,0.043137,0.043137);
rgb(245pt)=(0.039216,0.039216,0.039216);
rgb(246pt)=(0.035294,0.035294,0.035294);
rgb(247pt)=(0.031373,0.031373,0.031373);
rgb(248pt)=(0.027451,0.027451,0.027451);
rgb(249pt)=(0.023529,0.023529,0.023529);
rgb(250pt)=(0.019608,0.019608,0.019608);
rgb(251pt)=(0.015686,0.015686,0.015686);
rgb(252pt)=(0.011765,0.011765,0.011765);
rgb(253pt)=(0.007843,0.007843,0.007843);
rgb(254pt)=(0.003922,0.003922,0.003922);
rgb(255pt)=(0.000000,0.000000,0.000000);
}
}

==> figures/primal_dual_mesh/mesh_colors.tex <==
\colorlet{primalcolor}{gray!50!green}
\colorlet{dualcolor}{gray!50!white}
\colorlet{primalcolorhigh}{primalcolor!80!black}
\colorlet{dualcolorhigh}{dualcolor!80!black}
\colorlet{evalcolor}{gray!50!red}

==> figures/primal_dual_mesh/mesh_macros.tex <==
%\colorlet{primalcolor}{gray!50!green}
%\colorlet{dualcolor}{gray!50!white}
%\colorlet{primalcolorhigh}{primalcolor!80!black}
%\colorlet{dualcolorhigh}{dualcolor!80!black}

\tikzset{coord/.style={draw=none, inner sep=0pt}}
\tikzset{subdue/.style={opacity=1.}}
\tikzset{primalhigh/.style={draw=primalcolorhigh, ultra thick}}
\tikzset{dualhigh/.style={draw=dualcolorhigh, ultra thick}}
\tikzset{primal/.style={draw=primalcolor}}
\tikzset{dual/.style={draw=dualcolor}}
\tikzset{primal face/.style={primal,thin,solid}}
\tikzset{dual face/.style={dual,thin,solid}}
\tikzset{primal vertex/.style={fill=primalcolor,minimum size=0.032*\figurewidth,inner sep=0pt,circle}}
\tikzset{dual vertex/.style={fill=dualcolor,minimum size=0.032*\figurewidth,inner sep=0pt,rectangle}}
\tikzset{primal face midpoint/.style={fill=primalcolor,minimum size=0.005*\figurewidth,inner sep=0pt,circle}}
\tikzset{primal cell/.style={draw=primalcolor, fill=primalcolor, opacity=0.2}}
\tikzset{dual cell/.style={draw=dualcolor, fill=dualcolor, opacity=0.2}}
%\tikzset{cell/.style={thick,solid,opacity=1}}


%\def\makemeshpair#1#2{
%	% define and draw primal vertices
%	\foreach \pj/\px/\py in {#1}
%	{
%		\path (\px*\figurewidth,\py*\figureheight) node[primal vertex](pvert\pj) {}; 
%	}
%	%loop over primal cells. each tuple is the cell name an\textit{}d the three vertices
%	\foreach \dr/\pj/\pk/\pl in {#2} 
%	{
%		% draw primal faces and define and draw face midpoints
%		\path[primal face] (pvert\pj) -- node[midway, primal face midpoint](pfacemid\pj\pk){} node[coord, midway] (pfacemid\pk\pj) {} (pvert\pk); 
%		\path[primal face] (pvert\pj) -- node[midway, primal face midpoint](pfacemid\pj\pl){} node[coord, midway] (pfacemid\pl\pj) {} (pvert\pl); 
%		\path[primal face] (pvert\pk) -- node[midway, primal face midpoint](pfacemid\pk\pl){} node[coord, midway] (pfacemid\pl\pk) {} (pvert\pl); 
%		% define and draw cell centers/ dual vertices
%		\path ($ 0.3333333*($ (pvert\pj) + (pvert\pk) + (pvert\pl) $)$)node[dual vertex] (dvert\dr) {}; 
%		% draw dual faces between primal cell midpoint and all contributing edge centers 
%		\path[dual face] (dvert\dr) -- (pfacemid\pj\pk);
%		\path[dual face] (dvert\dr) -- (pfacemid\pj\pl);
%		\path[dual face] (dvert\dr) -- (pfacemid\pk\pl);
%	}
%}

\def\makemeshpair#1#2#3{
	% define and draw primal vertices
	\foreach \pj/\px/\py in {#1}
	{
		\path (\px*\figurewidth,\py*\figureheight) node[primal vertex](pvert\pj) {}; 
	}
	%loop over primal triangle cells. each tuple is the cell name and the three vertices
	\foreach \dr/\pj/\pk/\pl in {#2} 
	{
		% draw primal faces and define and draw face midpoints
		\path[primal face] (pvert\pj) -- node[midway, primal face midpoint](pfacemid\pj\pk){} node[coord, midway] (pfacemid\pk\pj) {} (pvert\pk); 
		\path[primal face] (pvert\pj) -- node[midway, primal face midpoint](pfacemid\pj\pl){} node[coord, midway] (pfacemid\pl\pj) {} (pvert\pl); 
		\path[primal face] (pvert\pk) -- node[midway, primal face midpoint](pfacemid\pk\pl){} node[coord, midway] (pfacemid\pl\pk) {} (pvert\pl); 
		% define and draw cell centers/ dual vertices
		\path ($ 0.3333333*($ (pvert\pj) + (pvert\pk) + (pvert\pl) $)$)node[dual vertex] (dvert\dr) {}; 
		% draw dual faces between primal cell midpoint and all contributing edge centers 
		\path[dual face] (dvert\dr) -- (pfacemid\pj\pk);
		\path[dual face] (dvert\dr) -- (pfacemid\pj\pl);
		\path[dual face] (dvert\dr) -- (pfacemid\pk\pl);
	}
	%loop over primal quadrilaterals. each tuple is the cell name and the three vertices
	\foreach \dr/\pj/\pk/\pl/\pm in {#3} 
	{
		% draw primal faces and define and draw face midpoints
		\path[primal face] (pvert\pj) -- node[midway, primal face midpoint](pfacemid\pj\pk){} node[coord, midway] (pfacemid\pk\pj) {} (pvert\pk); 
		\path[primal face] (pvert\pk) -- node[midway, primal face midpoint](pfacemid\pk\pl){} node[coord, midway] (pfacemid\pl\pk) {} (pvert\pl); 
		\path[primal face] (pvert\pl) -- node[midway, primal face midpoint](pfacemid\pl\pm){} node[coord, midway] (pfacemid\pm\pl) {} (pvert\pm);
		\path[primal face] (pvert\pm) -- node[midway, primal face midpoint](pfacemid\pm\pj){} node[coord, midway] (pfacemid\pj\pm) {} (pvert\pj);  
		% define and draw cell centers/ dual vertices
		\path ($ 0.25*($ (pvert\pj) + (pvert\pk) + (pvert\pl) + (pvert\pm) $)$)node[dual vertex] (dvert\dr) {}; 
		% draw dual faces between primal cell midpoint and all contributing edge centers 
		\path[dual face] (dvert\dr) -- (pfacemid\pj\pk);
		\path[dual face] (dvert\dr) -- (pfacemid\pk\pl);
		\path[dual face] (dvert\dr) -- (pfacemid\pl\pm);
		\path[dual face] (dvert\dr) -- (pfacemid\pm\pj);
	}
}

\def\markdualcell#1#2#3#4{%
	\path[dual cell, #4]
	(dvert#2.center) 
	\foreach \facemid/\dr in {#3} 
	{
		 -- (pfacemid#1\facemid.center) -- (dvert\dr.center)
	}
	-- cycle; 
}


\def\gridspacing{0.2*\figurewidth}
\def\pvertex#1#2{(#1*\gridspacing,#2*\gridspacing)}
\def\dvertex#1#2{($ (#1*\gridspacing,#2*\gridspacing) - (0.5*\gridspacing,0.5*\gridspacing)$)}
\def\pcell#1#2#3%
{%
	\draw[#3] let \n1={#1-1}, \n2={#2-1} in \pvertex{\n1}{\n2} rectangle\pvertex{#1}{#2};%
}
\def\dcell#1#2#3%
{%
	\draw[#3] let \n1={#1-1}, \n2={#2-1} in \dvertex{#1}{#2} rectangle\dvertex{\n1}{\n2};%
}
\def\psubcells#1#2#3%
{%
	\draw[#3] \dvertex{#1}{#2} ++ (-0.5*\gridspacing,0) -- ++(\gridspacing, 0); 
	\draw[#3] \dvertex{#1}{#2} ++ (0, -0.5*\gridspacing) -- ++(0, \gridspacing); 
}
\def\sgrid#1#2#3%
{	
	\foreach \xx in {1,...,#1}
	{
		\foreach \yy in {1,...,#2}
		{
			\path \dvertex{\xx}{\yy} coordinate(#3dvert\xx\yy);
		}
	}	
	
	\foreach \xx in {0,...,#1}
	{
		\foreach \yy in {0,...,#2}
		{
			\path \pvertex{\xx}{\yy} coordinate (#3pvert\xx\yy);
		}
	}
	
	\foreach \xx in {0,...,#1}
	{
		\foreach \yy in {0,...,#2}
		{
			\path (#3pvert\xx\yy) node[primal vertex] {}; 
%			\dcell{\xx}{\yy}{dual face}
		}
	}

	\foreach \xx in {1,...,#1}
	{
		\foreach \yy in {1,...,#2}
		{
			\path (#3dvert\xx\yy) node[dual vertex] {}; 
			\pcell{\xx}{\yy}{primal face}
			\psubcells{\xx}{\yy}{dual face}
%			\path [dual face] let \n1={\xx-1}, \n2={\yy-1}
		}
	}
		

	
}

==> postercolors.tex <==
\usepackage{xcolor}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% colors
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% general colors
\colorlet{alert}{red!80!black}
\colorlet{subdue}{black!80!white}

%% TUK colors
%
\definecolor{tuklblue}{RGB}{0,95,140}
\definecolor{tuklred}{RGB}{185,40,25}
\definecolor{tuklcoldgray}{RGB}{130,125,120}
\definecolor{tuklwarmgray}{RGB}{130,140,150}
%
\definecolor{tuklmathematik}{RGB}{254,192,0}

%% poster colors
\colorlet{background1}{white}
\colorlet{background2}{background1}
\colorlet{header1}{tuklblue!25}
\colorlet{header2}{header1}
\colorlet{headerfont1}{black}
\colorlet{border1}{header1}
\colorlet{box1}{tuklblue!2!white}
\colorlet{box2}{box1}

%% emphasis background color
\colorlet{emph}{tuklblue!10!white}
